AnoShift: A Distribution Shift Benchmark for Unsupervised Anomaly Detection

Analyzing the distribution shift of data is a growing research direction in nowadays Machine Learning (ML), leading to emerging new benchmarks that focus on providing a suitable scenario for studying the generalization properties of ML models. The existing benchmarks are focused on supervised learning, and to the best of our knowledge, there is none for unsupervised learning. Therefore, we introduce an unsupervised anomaly detection benchmark with data that shifts over time, built over Kyoto-2006+, a traffic dataset for network intrusion detection. This type of data meets the premise of shifting the input distribution: it covers a large time span ($10$ years), with naturally occurring changes over time (eg users modifying their behavior patterns, and software updates). We first highlight the non-stationary nature of the data, using a basic per-feature analysis, t-SNE, and an Optimal Transport approach for measuring the overall distribution distances between years. Next, we propose AnoShift, a protocol splitting the data in IID, NEAR, and FAR testing splits. We validate the performance degradation over time with diverse models, ranging from classical approaches to deep learning. Finally, we show that by acknowledging the distribution shift problem and properly addressing it, the performance can be improved compared to the classical training which assumes independent and identically distributed data (on average, by up to $3\%$ for our approach). Dataset and code are available at https://github.com/bit-ml/AnoShift/.

==> __including_logs.tex <==
% \documentclass{article}

% % if you need to pass options to natbib, use, e.g.:
% \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_data_2022

% % ready for submission
% \usepackage{neurips_data_2022}

% % to compile a preprint version, add the [preprint] option, e.g.:
% % \usepackage[preprint]{neurips_data_2022}
% % This will indicate that the work is currently under review.

% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_data_2022}

% % to avoid loading the natbib package, add option nonatbib:
% % \usepackage[nonatbib]{neurips_data_2022}

% % Submissions to the datasets and benchmarks are typically non anonymous,
% % but anonymous submissions are allowed. If you feel that you must submit 
% % anonymously, you can compile an anonymous version by adding the [anonymous] 
% % option, e.g.:
% %     \usepackage[anonymous]{neurips_data_2022}
% % This will hide all author names.

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{amsmath}

% % adaugate de noi
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{makecell}
% \usepackage[symbol]{footmisc}
% \newcommand{\eg}{\textit{e}.\textit{g}. }

% % \title{A Streaming Protocol for Unsupervised Anomaly Detection}
% \title{Temporal Distribution Shift Benchmark for Targeting Anomalies}

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.

% \author{%
%   Marius Dragoi$^*$\\
%   Bitdefender, Romania\\
% %   \texttt{mdragoi@bitdefender.com} \\
%   \And
%   Elena Burceanu$^*$ \\
%   Bitdefender, Romania \\
%   University of Bucharest\\
% %   \texttt{mdragoi,eburceanu,ehaller@bitdefender.com} \\
%   \And
%   Emanuela Haller$^*$ \\
%   Bitdefender, Romania \\
%   Politehnica University of Bucharest\\
% %   \texttt{ehaller@bitdefender.com} \\
%   \And
%   Andrei Manolache \\
%   Bitdefender, Romania \\
% %   \texttt{amanolache@bitdefender.com} \\
%   \And
%   Florin Brad \\
%   Bitdefender, Romania \\
% %   \texttt{amanolache,fbrad@bitdefender.com} \\
% }




% % \author{%
% %   David S.~Hippocampus\thanks{Use footnote for providing further information
% %     about author (webpage, alternative address)---\emph{not} for acknowledging
% %     funding agencies.} \\
% %   Department of Computer Science\\
% %   Cranberry-Lemon University\\
% %   Pittsburgh, PA 15213 \\
% %   \texttt{hippo@cs.cranberry-lemon.edu} \\
% %   % examples of more authors
% %   % \And
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% %   % \AND
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% %   % \And
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% %   % \And
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% % }


% \begin{document}

% \maketitle

% \begin{abstract}
%   Continuous monitoring of IT infrastructure has become an important process of computer security and resilience. One of the key tools of this process is log-based anomaly detection. Recent anomaly detection (AD) and intrusion detection systems (IDS) are able to obtain very strong results on several datasets. However, their success is heavily influenced by several experimental setup decisions, which may lead to performance inconsistencies. Moreover, we argue that the common assumptions regarding the data distribution do not take into account the distribution shifts over time, leading to inflated scores on the test set. Specifically, we observe that the test performance of log-based anomaly detectors degrades with longer time horizons. To better assess the models' capabilities, we propose a streaming evaluation protocol, in which we distinctly evaluate anomalies that happen close to the training points versus anomalies that are more distant in the future.
% \end{abstract}

% unghiul 1:
% 1. distr shift ca important problem in ML
% 2. nids/logs ca dataset perfect pt asta (evolueaza peste timp, se schimba distr natural) 

% unghiul2:
% 1. taskul de anomaly detection in nids/logs care nu merg in real world scenario 
% 2. distr shift ca problema de fond a abordarilor


% 3 la ambele. Posibilitatea de metode pt time series multivariate


% Povestea:
% multe nids/logs metode (inclusiv cele clasice) si datasets saturate, in perspectiva supervised + iid, dar many si unsup. but in real world scenario nu merg, pentru ca datele se schimba. si problema nu e neaparat in dataset, ci in modul in care il folosim. nu yet another dataset, but a new way of seeing the problem. identificam la root problema, ca datele se schimba si propunem un benchmark (bazat pe datasets pe care le-am filtrat dintre mutlii candidati - pe suficient timespan, cu date reale nu fake - aproape de real world scenario, diferite procente de anomalii). testam variate metode (atat clasice cat si noi-transformer bert sa vedem care e performanta si mai ales daca se mentine cu trecerea timpului)



% \section{Introduction}
% \footnotetext{$^*$ Equal contribution. Bitdefender Theoretical Research Team: \url{https://bit-ml.github.io/}}

% % Most of the current methods naively split the training and the testing data, masking this long term horizon issue.

% % KEY ingredients for log-anomaly detector:
% % - unsupervised
% % - online 
% % - distribution shift -aware

% Performance of anomaly detectors on logs can vary significantly based on a number of training and preprocessing decisions. For instance, most of the current methods split the datasets such that train and test data are iid, leading to potential inflated performance due to training data containing example from the 'future'. Splitting the train/test sets such that chronological order is ensured (test events happen after the training events) leads to worse results \cite{Le2022} across several models. This confirms the iid splitting issue and suggests that more careful dataset preprocessing is needed to truly assess the log-based anomaly detectors' performance over larger time horizons (domain shift?). To this end, we propose a streaming evaluation protocol, inspired by the CLEAR benchmark \cite{clear}, which should better reflect the models' capabilities when dealing with distribution shifts across time.

% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.99\textwidth]{images/chronology.png}
%     \end{center}
%     \caption{\answerTODO{OUTDATED. Chronology protocol for evaluating iid versus \texttt{NEAR} and \texttt{FAR} splits}}
%     \label{fig:chronology}
% \end{figure}

% %nu-mi place cum e descris protocolul, dar e v1
% We illustrate in Fig.~\ref{fig:chronology} the splitting process on the Kyoto dataset, which spans several years of logs. Our splitting process can be adapted to different time windows (month, week etc.). We select a time period (2006-2010) and split it into train and test to obtain iid splits. We then select a time period adjacent to the training data (2011-2012), which we call \texttt{NEAR}. This \texttt{NEAR} subset is used for testing only and should reveal potential performance degradation when compared to the test iid set. We then select a time period which starts after the end timestamp of the \texttt{NEAR} subset plus a gap. We call this subset \texttt{FAR} and we expect models to exhibit the worse performance on the it. The results show the  model's progressive degradation from iid data to \texttt{NEAR} data, as well as further worsening from \texttt{NEAR} to \texttt{FAR}. 

% \paragraph{IID training vs Chronological methodology}

% \paragraph{Why Network Traffic and System Logs datasets?} Perfect for noticing distribution shifts, as they naturally change over time (what changes: one user network interaction (interest change), users, system interaction patterns, system/software versions=protocols).




% \paragraph{Our main contributions are:}
% \begin{itemize}
%     \item We propose a chronology-based splitting protocol, which distinguishes between iid test data, test data whose time is close to the iid test (\texttt{NEAR}) and distant test data (\texttt{FAR}).
%     \item We demonstrate based on the previous splits that the models' performance degrades over time and that the proposed iid, NEAR and FAR splits better reflect the true capabilities of log-anomaly detectors over distribution shifts. + propus pt evaluare de acum, pentru comparatii mai aproape de real world scenarios.
%     \item We treat the log-anomaly detection and intrusion detection in network traffic homogeneously and demonstrate the previous results on relevant datasets for both tasks.
% \end{itemize}


% \section{Related Work}

% \paragraph{WRT NIDS Anomalies} Modele foarte slabe...(rant despre cum modelele care fac IDS trateaza problema ca pe o problema de clasificare, ceea ce nu e posibil intr-un scenariu realist); 

% tree-based algorithms~\cite{tree}
% survey by anomaly types/methods~\cite{nids-survey, nids_survey_3, nids_survey_4}

% ensemble of autoencoder-based NIDS~\cite{ensemble_autoenc_nids}


% experiments on saturated data, compare shallow cu slightly  deep NNs, achieving similar results ~\cite{shallow_deep_nids}

%  A literature review in the area of anomaly detection with deep learning is beyond our purpose, there are already comprehensive surveys on anomalies (including Network Intrusion)~\cite{DL_anom_survey}
 
% to GNNs pt NIDS~\cite{gnn_nids}

% classic methods, multiple smaller datasets (inlcuding 3 years of kyoto), iid supervised training, large scores~\cite{compare_nids}.

% to images + CNN for feature extraction+SVM, saturated performance iid~\cite{nids_images_svm}


% (pe NIDS), modelele nu generalizeaza (huge drop in performance on newer/different datasets)~\cite{nids_generalization}

% % \paragraph{WRT LOGS Anomalies} ...Modele bunicele/uptodate,
% % arhitectura vs scorul de anomalie; sup vs unsup

% % A2Log~\cite{a2log}
% % CatLog~\cite{catlog} - bert+vae for feature extraction + contrastive adversarial training
% % LAnoBERT~\cite{lanobert}.


% % transformer-based~\cite{logbert, logsy}
% % lstm-based approaches~\cite{deeplog, loganomaly, robust_log_bert, nids_bilstm}, 
% % RNN+attention+computer system and logging source~\cite{rnn-logs}

% % A literature review in the area of anomaly detection with deep learning is beyond our purpose, there are already comprehensive surveys on anomalies (including System Logs and Network Intrusion)~\cite{DL_anom_survey}

% \paragraph{WRT Temporal Anomalies} ...

% \paragraph{WRT Online Learning/Continuous Learning Benchmarks} Recently, there is an increased amount of effort and focus in this direction, several benchmarks emerging that emphasize the distribution shift that might appear in data, from various reasons: over time~\cite{clear, mind_the_gap}, over the spatial location (gps)~\cite{intel_cl_benck}, or over different characteristics for ~\cite{wilds} (a subset of location variation). Nevertheless, those data focuses only on NLP or CV


% WILDS benchmark~\cite{wilds} (multi domain: NLP, CV, distr shift but not from temporal perspective)

% CLEAR benchmark~\cite{clear} (continual learning, over time, similar but in CV)

% CV benchmark~\cite{intel_cl_benck} benchmark for online continual visual learning that exhibits large scale and natural distribution shifts (gps data)

% NLP benchmark~\cite{mind_the_gap} (mind the gap)


% \section{Chrono-Protocol}

% \paragraph{TRAIN, NEAR, FAR splits} To emphasize the decrease in performance of models when dealing with temporarily distant data from the training set, we merge different splits over multiple datasets: yearly on the Kyoto-2006\texttt{+}, \answerTODO by semester/quarter in A, and by month in B. We also tested the degradation over a dataset with hour level splits (HDFS~\cite{hdfs}), but we obtained noisy results and conclude that for logs, the shift from hour to hour is mostly related to seasonality of a day. We create two separate test sets for each dataset, one close to the training data: NEAR and one farther apart: FAR.  We expect models to exhibit a better performance on \texttt{NEAR} compared to \texttt{FAR}, which we experimentally prove in Tab.~\ref{tab:far_near}. We specify bellow the TRAIN, NEAR and FAR splits for each dataset, in its subsection and in Fig.~\ref{fig:counts}.

% \subsection{Network IDS}
% \subsubsection{Kyoto-2006\texttt{+}}
% Kyoto-2006\texttt{+}~\cite{kyoto2006} is a reference dataset for Anomaly Detection over network traffic data~\cite{}. It is build on 10 years of real traffic data (Nov. 2006 - Dec. 2015), captured in a system of 348 honeypots, in 5 sub-networks inside the Kyoto University. Briefly, a honeypot is a real or virtual machine simulating a normal computer (having an OS and multiple services running on it). Its purpose is to deceive an attacker to take advantage of the vulnerabilities that are present on the honeypot machine (\eg software not updated). When an attacker hits, the honeypot saves the network access pattern and other metadata and at some point might decide to reboot the system and rewrite back the original configuration. A honeypot does not request any connection by its own. So in such scenario, almost all traffic coming to a honeypot machine is unsolicited, therefore considered malicious. By design, this kind of datasets have a large percent of anomalies (89.5\% anomalies  in Kyoto-2006\texttt{+}) when compared with other anomaly detection datasets. For generating normal traffic data, the authors deployed another machine in the network, with a mailing server and a DNS service for a single domain. All traffic data from this server was labeled as clean (the logs includes also other protocols for managing the machine over ssh or http and https). The malicious traffic is further labeled using three software solutions: an Intrusion Detection Systems at network level, an Antivirus product, and a shellcodes and exploits detector. In addition to those, the authors labeled other entries based on their prior history of connections from a specific IP and destination port. Notice that this dataset spread across a very large time span and it contains exclusively real world  traffic events, without simulated events.

% % \begin{figure}[t]
% %     \begin{center}
% %         \includegraphics[width=0.5\textwidth]{images/dataset_characteristics.png}
% %     \end{center}
% %     \caption{\answerTODO{Datasets characteristic comparison between KDD99 and Kyoto-2006\texttt{+}}}
% %     \label{fig:kyoto_stats}
% % \end{figure}

% % \begin{figure}[t]
% %     \begin{center}
% %         \includegraphics[width=0.2\textwidth]{images/k1.png}
% %         \includegraphics[width=0.2\textwidth]{images/k2.png}
% %         \includegraphics[width=0.2\textwidth]{images/k3.png}
% %         \includegraphics[width=0.15\textwidth]{images/dataset_descr.png}
% %     \end{center}
% %     \caption{Kyoto labeling statistics}
% %     \label{fig:kyoto_stats2}
% % \end{figure}


% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=1\textwidth]{images/counts_kyoto.png}
%         % \includegraphics[width=1\textwidth]{images/counts_bgl_spirit.png}
%         % \includegraphics[width=0.2\textwidth]{images/k3.png}
%         % \includegraphics[width=0.15\textwidth]{images/dataset_descr.png}
%     \end{center}
%     \caption{Number of samples. First line: before and after our splitting for Kyoto, that fixes the number of normal samples between splits, while keeping the anomaly vs normal proportion in each split. BGL and Spirit splits on the second row.}
%     \label{fig:counts}
% \end{figure}

% \paragraph{Splitting by year} Our splitting is straight forward, mapped on the original dataset proposal: we divide the dataset into years, and keep the number of normal samples proportional with the time span for which we have data in each year. As for the anomaly samples, we maintain the percent that we find in the original data, as shown in Fig.~\ref{fig:counts}a. (\eg 2006 contains only 2 months while the other years have data for all 12 month, so we keep 6x more clean samples in other years wrt 2006). We argue that by splitting the dataset in this way, we firstly do not introduce biases tailored for a specific period like in the original setup, and, secondly, we do not interfere with the anomalous vs normal proportion found in the real data. The \textbf{TRAIN} split consists of interval [2006, 2010], \textbf{NEAR} [2011, 2013], and \textbf{FAR} [2014, 2015], like shown in Fig.~\ref{fig:counts}.


% \paragraph{Preprocess network traffic data} We use the 14 conventional features from the new version of the Kyoto dataset (2006-2015), which consists of two categorical features: connection service type and flag of the connection and 12 numerical features: duration of the connection, number of source and destination bytes, number of connections with corresponding IP addresses in a timeframe of two seconds and the percentage of connections accessing the same service and their rate of "SYN" errors, the prevalence of the connection's soruce IP address and the requested service in the past 100 connections to the current destination IP. We convert the numerical features to categorical ones by using an exponential-scaled binning method between 0 and the maximum value ($2^{32} -1$) of each feature, such that the bins have a higher density for smaller numerical values and are increasingly larger towards larger values. We used a basis of 1.1, which resulted in 233 bins, where the width of bin i is given by:
% \begin{equation}
%     bin_i = [1.1^{i} - 1, 1.1^{i+1} -1]
% \end{equation}
% The numerical features denoting percents are already discretized in 100 distinct values. Therefore, our preprocessing results in a fixed vocabulary size for the language models, where each possible token is known apriori. A sample of preprocessed instances is shown in Figure \ref{fig:kyoto_instance}.


% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=1.0\textwidth]{images/kyoto_sample.png}
%     \end{center}
%     \caption{Kyoto-2006 sample of preprocessed instances}
%     \label{fig:kyoto_instance}
% \end{figure}


% \subsection{System Logs}

% \subsubsection{BGL}
% \paragraph{Splitting by ...}

% \subsubsection{Spirit}
% \paragraph{Splitting by ...}


% \paragraph{Preprocess system logs data}  \answerTODO{Drain/Spell}

% % \subsubsection{Thunderbird}
% % \paragraph{Splitting by ...}
% \subsection{BERT for Anomalies} We propose a simplified BERT architecture for detecting anomalies. The network input is tokenized by a WordLevel tokenizer which obtains tokens for the individual events in a system log sequence and, conversely, for the individual features of network traffic. Therefore, we have variable-length sequences for system logs and fixed-length sequences for Kyoto-2006. We train the BERT model as a Masked Language Model (MLM), using a data collator that randomly masks p\% of the input sequence, by optimizing a cross-entropy loss function between the model predictions at mask positions and the original tokens. We derive a sequence anomaly score by randomly masking p\% of tokens in the sequence and averaging the probabilities of the correct tokens at mask positions given by the classification layer over the vocabulary. 

% \begin{equation}
%     \hat{w_j}^i =  \begin{cases}
%                         w_j, & \text{if $mask_i$(j) = 0} \\
%                         [MASK], & \text{if $mask_i$(j) = 1}
%                     \end{cases}
%     \label{masking}
% \end{equation}

% We repeat the masking process n times and average over all repeats to improve consistency. The anomaly score formula is depicted in equation \ref{anom_score}, where we denote by $P_M$ the classification layer of the model of parameters $\theta_M$, by $Masks^{p}_{k}$ the set of random binary masks of length k and mask probability p, where $w_t$ are the initial tokens in the sequence and $\hat{w_t}^i$ is the j-th token in the sequence under mask i.

% \begin{equation}
% anomaly\_score([w_1, w_2, ... , w_t]) = \frac{\sum_{i=1..n} \sum_{j=1..t}^{mask_i \sim Masks^{p}_t} (1 - P(\hat{w_j}^i)) }{n}
% \label{anom_score}
% \end{equation}


% \begin{equation}
%     P(\hat{w_j}^i) =  \begin{cases}
%                         1, & \text{if $mask_i$(j) = 0} \\
%                         P_M(w_j | \theta_M, [\hat{w_1}^i, ..., \hat{w_t}^i]), & \text{if $mask_i$(j) = 1}
%                     \end{cases}
%     \label{classif_prob}
% \end{equation}

% We motivate this metric with the observation that inlier data should consist of common tokens with a high retrieval probability given by the distribution of the training set, while outliers should usually have either rare tokens or unusual combinations of features, within the context given by the unmasked tokens. 


% \section{Experimental Analysis}


% \paragraph{Baselines} For better analysing the variation of datasets distribution over time, we tested the performance of several unsupervised baselines, ranging from classic approaches like Isolation Forest~\cite{isoforest} and OC-SVM~\cite{ocsvm} to newer ones based on modeling the input data as language models: DeepLog~\cite{deeplog} and LogAnomaly~\cite{loganomaly} based on LSTMs~\cite{lstm}, and, LogBERT~\cite{logbert} and our proposed transformer for anomalies model, both based on the BERT architecture. We test these baselines in a wide variety of scenarios as describe next in this section.

% \paragraph{Our BERT} We use a simplified BERT architecture, without pretraining, consisting of two hidden layers of size $120$, an intermediate size of $192$ and $6$ attention heads. It has a hidden dropout and attention dropout probabilities of $0.1$, an epsilon of $1e-12$ for the normalization layer and a $0.02$ standard deviation range for the truncated normal weight initialization. Our architecture totals $342135$ trainable parameters. For training we mask $p=15\%$ of the input sequence and at evaluation time, we average over $n=10$ masking samplings.

% \paragraph{Metrics for Anomaly Detection} Since we discuss datasets splits that have labels and are highly unbalanced, ROC-AUC is the fair metric to use for comparing the performance in different scenarios. For better understanding the problems with different splits and models, we also report the Precision-Recall-AUC both for inliers and outliers in the appendix \answerTODO{}, but only for analysis, since this metric is highly unstable when the data proportion changes. Please note that for a random classifier, PR-AUC for a specific class is close to 0.



% \subsection{Chrono vs iid - the illusion of high performance}
% Tab.~\ref{tab:far_near} 


% \begingroup
% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \begin{table}[t]
% \begin{center}
%     \caption{Performance gap over time: NEAR vs FAR on each dataset. We report ROC-AUC in the table, and add the PR-AUC to the appendix....}
%         \begin{tabular}{m{3em} c l c c c}
        
%         \toprule
%         & & & \multicolumn{4}{c}{ROC-AUC $\uparrow$}\\
%         \cmidrule{4-7}
%         \textbf{Dataset} & \textbf{Parser} & \textbf{Split} & \textbf{our BERT} & \textbf{OC-SVM} & \textbf{IsoForest}\\
%         \midrule
%         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\makecell{Network\\\textbf{Kyoto}}}}}
%         &  & \textbf{TRAIN} &   $\pm$ \small  & 86.82 $\pm$ \small 0 & 66.93 $\pm$  \small 4.62\\
%         & log & \textbf{NEAR} & 78.42 $\pm$ \small  & 71.06 $\pm$ \small 0 & 41.20 $\pm$ \small 9.60\\
%         &  Binning & \textbf{FAR} & 49.16 $\pm$ \small  & 41.42 $\pm$ \small 0 & 18.47 $\pm$ \small 2.68\\
%         \midrule
        
%         %  &  & &  & \textbf{LogBERT}\cite{logbert} & \textbf{DeepLog} \cite{deeplog} & \textbf{LogAnomaly} \cite{loganomaly} & \textbf{PCA}\\
%         % \midrule
%         % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\makecell{Logs\\\textbf{BGL}}}}}
%         % &  & \textbf{TRAIN} &  50.50 $\pm$ \small  & 98.23 $\pm$ \small & 67.34 $\pm$ \small & 67.35 $\pm$ \small\\
%         % & Spell & \textbf{NEAR} &  38.6 $\pm$ \small  & 13.79 $\pm$ \small & 43.22 $\pm$ \small & 42.03 $\pm$ \small\\
        
%         % &  & \textbf{FAR} &  41.2 $\pm$ \small  & 7.08 & 45.08$\pm$ \small & 45.13 $\pm$ \small\\
%         % \cmidrule{3-7}
%         % &  & \textbf{TRAIN} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
%         % & Drain & \textbf{NEAR} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
%         % &  & \textbf{FAR} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
      
%         % \midrule
        
%         % \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\makecell{Logs\\\textbf{Spirit}}}}}
%         % &  & \textbf{TRAIN} &  $\pm$ \small  & 87.45 $\pm$ \small & 80.32 $\pm$ \small & 80.28 $\pm$ \small\\
%         % & Spell & \textbf{NEAR} & 56.41 $\pm$ \small  & 42.52 $\pm$ \small & 63.19 $\pm$ \small & 63.73$\pm$ \small\\
%         % &  & \textbf{FAR} &  79.32$\pm$ \small  & 70.91 $\pm$ \small & 75.01 $\pm$ \small & 75.09 $\pm$ \small\\
%         % &  & \textbf{SEZON} &  77.25$\pm$ \small  & 78.02 $\pm$ \small & 77.22 $\pm$ \small & 77.17$\pm$ \small\\
%         % \cmidrule{3-7}
%         % &  & \textbf{TRAIN} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
%         % & Drain & \textbf{NEAR} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
%         % &  & \textbf{FAR} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
%         % &  & \textbf{SEZON} &  $\pm$ \small  & $\pm$ \small & $\pm$ \small\\
        
%         \bottomrule
%         \end{tabular}
% \end{center}
% \label{tab:far_near}
% \end{table}
% \endgroup



% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat1.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat2.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat3.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat9.png}
%     \end{center}
%     \caption{Jeffreys divergence between Kyoto years for features with a large 
%     2014-2015 distance.}
%     \label{fig:jeff_kyoto}
% \end{figure}

% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat4.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat10.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat6.png}
%         \includegraphics[width=0.23\textwidth]{images/jeff_feat7.png}
%     \end{center}
%     \caption{Jeffreys divergence between Kyoto years for other features. Note that it is hard to say in advance what will be the performance of the method on a new split, only based on those per feature distances between distributions.}
%     \label{fig:jeff_kyoto_others}
% \end{figure}
% \subsection{Distribution shift analysis}

% \subsubsection{Per feature shift}
% \subsubsection*{Kyoto - discrepancies} 
% We further analyse whether the statistics of the dataset at feature level is changing from one year to another. Recall that we have 2 categorical features and 11 numerical ones. For each feature, we extract the normalized histogram per year and compute the Jeffreys divergence~\cite{jeff_divergence} between those histograms. The Jeffreys divergence is a commonly used symmetrization for KL~\cite{kl_divergence}: $KL(p, q) + KL(q, p)$, and it is proven to be both symmetric and non-negative. We present next in this section, this kind of analysis, but note that it only highlights simple cases, when it is easy to see that a distribution is changed based on a single feature. We analyze further in Sec.~\ref{sec: otdd} the dataset from a more general point of view, which also takes into account the combinations of the input features, analysing discrepancies in latent space.

% \paragraph{2014+2015} With all tested baselines, we notice a significant decrease in performance for 2014-2015 years for inliers (even below the random performance), showing that there might be a particularity with those years. We observe a large distance in the above described distances for 4 features (service type, connection duration, packet size and same source-destination pairs count) between the 2014-2015 years and all the rest (see Fig.~\ref{fig:jeff_kyoto}). One root cause of those events can be the increasing of the "DNS" traffic (from 12\% to 22\% and 14\% of the total traffic, in 2013, 2014 and 2015 respectively) for the inliers class, samples that become miss-classified as we experimentally tested?. \answerTODO{experiment sa demonstreze explicit asta}. More, see the same analysis for other features in Fig.~\ref{fig:jeff_kyoto_others} that highlights the fact that it is hard to predict the performance on a split, just given the per feature distances between distributions.

% % \paragraph{2009+2010} \answerTODO{daca mai e cazul la BERT/OC-SVM (in noile isoforest nu se vede nimic)}


% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.31\textwidth]{images/otdd_kyoto_5k_inliers.png}
%         \includegraphics[width=0.31\textwidth]{images/otdd_kyoto_5k_inliers+outliers.png}
%         \includegraphics[width=0.32\textwidth]{images/otdd_kyoto_5k_outliers.png}
%     \end{center}
%     \caption{Optimal Transport Dataset Distance for Kyoto. See distances only between inliers in the first image, between both inliers and outliers in the second, and outliers only in the third. You can notice how groups of years that are similar with each other (dark color), are gradually distant from others (2007+2008, 2008+2009, 2011+2012+2013, 2014+2015 - first image). See how the distances generally increase as you move further from the diagonal.}
%     \label{fig:otdd_kyoto}
% \end{figure}

% % \begin{figure}[t]
% %     \begin{center}
% %         \includegraphics[width=0.31\textwidth]{images/otdd_bgl_5k_inliers_Drain.png}
% %         \includegraphics[width=0.31\textwidth]{images/otdd_bgl_5k_inliers+outliers_Drain.png}
% %         \includegraphics[width=0.32\textwidth]{images/otdd_bgl_5k_outliers_Drain.png}
        
% %         \includegraphics[width=0.31\textwidth]{images/otdd_bgl_5k_inliers_Spell.png}
% %         \includegraphics[width=0.31\textwidth]{images/otdd_bgl_5k_inliers+outliers_Spell.png}
% %         \includegraphics[width=0.32\textwidth]{images/otdd_bgl_5k_outliers_Spell.png}
% %     \end{center}
% %     \caption{OTDD for BGL Drain+Spell: inliers, inliers+outliers, outliers.}
% %     \label{fig:otdd_bgl}
% % \end{figure}



% % \begin{figure}[t]
% %     \begin{center}
% %         \includegraphics[width=0.31\textwidth]{images/otdd_spirit_5k_inliers_Spell.png}
% %         \includegraphics[width=0.31\textwidth]{images/otdd_spirit_5k_inliers+outliers_Spell.png}
% %         \includegraphics[width=0.32\textwidth]{images/otdd_spirit_5k_outliers_Spell.png}
% %     \end{center}
% %     \caption{OTDD for Spirit Spell: inliers, inliers+outliers, outliers.}
% %     \label{fig:otdd_spirit}
% % \end{figure}



% \begin{figure}[t]
%     \begin{center}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2006-2007.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2007-2008.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2008-2009.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2009-2010.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2010-2011.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2011-2012.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2012-2013.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2013-2014.png}
%         \includegraphics[width=0.32\textwidth]{images/tsne_2014-2015.png}
%     \end{center}
%     \caption{Visual representation of the distribution shift for Kyoto splits - inliers only. Each plot represents the TSNE(RoboustScaller(input)) projection for two adjacent years. It is clear that the data distribution is not fix, since one can observe parts that do not overlap (have one color, belonging to a single year), showing how data shifts over time. Observe this figure in parallel with OTDD in Fig.~\ref{fig:otdd_kyoto}a: 2006-2007-2008 block seam quite similar (with large overlaps), next also 2009-2010, 2011-2012-2013, and 2014-2015 form other blocks with similar distributions. Larger differences can be seen at their borders, when plotting years belonging to different blocks.}
%     \label{fig:tsne_by_year}
% \end{figure}


% \subsubsection{General shift}
% \label{sec: otdd}
% We explore next the distribution differences between dataset splits over time, by using Optimal Transport Dataset Distance method (OTDD)~\cite{otdd}. OTDD relies on optimal transport, which is a geometric method for comparing the probability distributions, designed for comparing datasets. This analysis shows how the splits are moving away one from each other over time (see Fig.~\ref{fig:otdd_kyoto}). Compared with the per feature approach, this method allows us to gain a better intuition for the performance on a new split, giving us a single distance based on all features. We run the method with inner\_ot\_method='exact' and the default parameters for DatasetDistance, over the standardized input of Kyoto, with one-hot encoded categorical variables.



% % \subsubsection{Wider context}
% % In a wider context, \answerTODO{analizat chestia cu china+kyoto de la marvis}

% \subsection{Training strategies for data shift}

% Tab.~\ref{tab:training_strategies}
% \begin{table}[t]
% \caption{\answerTODO{Training strategies: IID train vs Finetune vs Distil on Kyoto-2006/other dataset (ROC-AUC presented - PR-AUC-in/out in appendix); poate plot}}
% \setlength{\tabcolsep}{7pt} % Default value: 6pt
% \begin{center}
% \begin{tabular}{l llllc llllc }

% \toprule
%  & \shortstack{Train ON: 2006->} & \multicolumn{1}{c}{\textbf{2007}} & \multicolumn{1}{c}{\textbf{2008}} & \multicolumn{1}{c}{\textbf{2009}} & \multicolumn{1}{c}{\textbf{2010}} \\ 
% \textbf{Strategy} & \shortstack{Split} \\
% \toprule

% \multicolumn{1}{l}{\textbf{IID}} & NEAR \\
% & FAR\\
% \midrule
% \multicolumn{1}{l}{\textbf{Finetune}} & NEAR \\
% & FAR \\
% \midrule
% \multicolumn{1}{l}{\textbf{Distil}}  & NEAR \\ 
% & FAR \\

% \bottomrule

% \end{tabular}
% \label{tab:training_strategies}
% \end{center}
% \end{table}



% \begin{table}[t]
% \caption{\answerTODO{transformat in plot}}
% \setlength{\tabcolsep}{7pt} % Default value: 6pt
% \begin{center}
% \begin{tabular}{l llllc  llllc }
%     \toprule
%      & \textbf{Outliers in train} & 0\% & 5\% & 10\% & 15\% & 20\% & 25\%\\ 
%     \textbf{Split} \\
%     \toprule
%     NEAR \\
%     FAR\\
%     \bottomrule
% \end{tabular}
% \label{tab:impure_train}
% \end{center}
% \end{table}

% \subsection{Impure training data}
% All our previous experiments are done training only on inliers. Here we test the resilience of our BERT baseline mislabeled outliers in the training data, under different percentages. See in Tab.~\ref{tab:impure_train} how its performance evolve in this scenario.





% \section{Discussions}
% \begin{itemize}
%     \item DISCUTIE pe faptul ca MLM nu e prea ok pt detectia de anomalii daca nu sunt corelate features intre ele
%     \item BERT models that uses only the train vocabulary - start seeing new events like UNK and this artificialy increase thier scores (la dataseturile pe loguri) - VEZI matricile de histograme de la ema cu si fara UNK
%     \item fake data vs natural gathered data (inliers fake and outliers natural si invers) - discutie per dataset
%     \item ploturi cu scorurile per split (an/luna/etc), nu direct TRAIN/NEAR/FAR
% \end{itemize}

% \section{Conclusions and Future Work}

% \answerTODO{recitit emailul de la razvan}

% \bibliographystyle{plainnat}
% \bibliography{neurips_benchmark}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~X.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

% \begin{enumerate}

% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerTODO{}
%   \item Did you describe the limitations of your work?
%     \answerTODO{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerTODO{}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerTODO{}
% \end{enumerate}

% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerTODO{}
% 	\item Did you include complete proofs of all theoretical results?
%     \answerTODO{}
% \end{enumerate}

% \item If you ran experiments (e.g. for benchmarks)...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerTODO{}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerTODO{}
% 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerTODO{}
% 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerTODO{}
% \end{enumerate}

% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerTODO{}
%   \item Did you mention the license of the assets?
%     \answerTODO{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerTODO{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerTODO{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerTODO{}
% \end{enumerate}

% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerTODO{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%     \answerTODO{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%     \answerTODO{}
% \end{enumerate}

% \end{enumerate}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \appendix

% \section{Appendix}

% Include extra information in the appendix. This section will often be part of the supplemental material. Please see the call on the NeurIPS website for links to additional guides on dataset publication.

% \begin{enumerate}

% \item Submission introducing new datasets must include the following in the supplementary materials:
% \begin{enumerate}
%   \item Dataset documentation and intended uses. Recommended documentation frameworks include datasheets for datasets, dataset nutrition labels, data statements for NLP, and accountability frameworks.
%   \item URL to website/platform where the dataset/benchmark can be viewed and downloaded by the reviewers.
%   \item Author statement that they bear all responsibility in case of violation of rights, etc., and confirmation of the data license.
%   \item Hosting, licensing, and maintenance plan. The choice of hosting platform is yours, as long as you ensure access to the data (possibly through a curated interface) and will provide the necessary maintenance.
% \end{enumerate}

% \item To ensure accessibility, the supplementary materials for datasets must include the following:
% \begin{enumerate}
%   \item Links to access the dataset and its metadata. This can be hidden upon submission if the dataset is not yet publicly available but must be added in the camera-ready version. In select cases, e.g when the data can only be released at a later date, this can be added afterward. Simulation environments should link to (open source) code repositories.
%   \item The dataset itself should ideally use an open and widely used data format. Provide a detailed explanation on how the dataset can be read. For simulation environments, use existing frameworks or explain how they can be used.
%   \item Long-term preservation: It must be clear that the dataset will be available for a long time, either by uploading to a data repository or by explaining how the authors themselves will ensure this.
%   \item Explicit license: Authors must choose a license, ideally a CC license for datasets, or an open source license for code (e.g. RL environments).
%   \item Add structured metadata to a dataset's meta-data page using Web standards (like schema.org and DCAT): This allows it to be discovered and organized by anyone. If you use an existing data repository, this is often done automatically.
%   \item Highly recommended: a persistent dereferenceable identifier (e.g. a DOI minted by a data repository or a prefix on identifiers.org) for datasets, or a code repository (e.g. GitHub, GitLab,...) for code. If this is not possible or useful, please explain why.
% \end{enumerate}

% \item For benchmarks, the supplementary materials must ensure that all results are easily reproducible. Where possible, use a reproducibility framework such as the ML reproducibility checklist, or otherwise guarantee that all results can be easily reproduced, i.e. all necessary datasets, code, and evaluation procedures must be accessible and documented.

% \item For papers introducing best practices in creating or curating datasets and benchmarks, the above supplementary materials are not required.
% \end{enumerate}



% \end{document}

